OORD: The Oxford Offroad Radar Dataset

There is a growing academic interest as well as commercial exploitation of millimetre-wave scanning radar for autonomous vehicle localisation and scene understanding. Although several datasets to support this research area have been released, they are primarily focused on urban or semi-urban environments. Nevertheless, rugged offroad deployments are important application areas which also present unique challenges and opportunities for this sensor technology. Therefore, the Oxford Offroad Radar Dataset (OORD) presents data collected in the rugged Scottish highlands in extreme weather. The radar data we offer to the community are accompanied by GPS/INS reference - to further stimulate research in radar place recognition. In total we release over 90GiB of radar scans as well as GPS and IMU readings by driving a diverse set of four routes over 11 forays, totalling approximately 154km of rugged driving. This is an area increasingly explored in literature, and we therefore present and release examples of recent open-sourced radar place recognition systems and their performance on our dataset. This includes a learned neural network, the weights of which we also release. The data and tools are made freely available to the community at https://oxford-robotics-institute.github.io/oord-dataset.

==> reply.tex <==
%------------------------------------------------------------------
% \todo[inline]{}

%------------------------------------------------------------------
\subsection*{Reviewer 1}

%------------------------------------------------------------------
\OB{1.1}{
Page 2 in the Introduction section: This paper primarily discusses the advantages of radar sensors. However, to provide a more comprehensive analysis, it is necessary to delve into the advantages and disadvantages of other advanced sensors such as cameras and LiDARs. By comparing these sensors, readers can better understand the rationale behind choosing radar sensors in this paper.
}
\REP{1.1}{
We have amended the manuscript as suggested, \fixRef{1.1}.
}

%------------------------------------------------------------------
\OB{1.2}{
Page 4 in Fig. 2 and Page 9 in Fig.6 Top Right: The top right figures show the ground truth matrix from GPS, which is challenging to connect with the GPS map figure, camera location figure, and the scanned radar figures. It is essential to provide more explanation about the significance of the white lines and dark black background in these figures.
}
%
\REP{1.2}{
We have done so -- \fixRef{1.2}.
}

%------------------------------------------------------------------
\OB{1.3}{
Page 6 in Fig. 5: Provide further explanation regarding “difference matrix”. The distance results in figures of baseline 2 and 3 closely resemble those in Fig. 2 and 6 Top Right, but why do the figures of baseline 1 and 8 appear so distinct? Because of using different matrix? And clarify the meaning of the grid representation in Fig. 5 (a) and (b).
}
%
\REP{1.3}{
For~\cref{fig:diff}, please see the edited manuscript at \fixRef{1.3.1}.
For the difference in difference matrices between \ref{B1} and \ref{B8}, please see~\fixRef{1.3.2}.
For~\cref{figs:diff_ringkey,figs:diff_alexnet}, please see a note added in~\fixRef{1.3.3}.
}

%------------------------------------------------------------------
\OB{1.4}{
Page 8 in the Examples section: Implementing nine different methods (baselines) in your dataset indicates that the proposed dataset is widely suitable for various networks. However, a thorough analysis is needed to explain why these specific nine pre-trained networks are chosen. Additionally, it would be valuable to provide insights into not only comparative results but also other performance metric such as the number of training parameters and training speed of each pre-trained networks.
}
%
\REP{1.4}{
We have add a robust justification for the choice of the pre-trained networks in~\fixRef{1.4.1} (with additional references added in~\fixRef{1.4.2}, \fixRef{1.4.3}, \fixRef{1.4.4}, \fixRef{1.4.6}).
There may be a slight misunderstanding in this comment, as there are not \textit{nine} pre-trained networks: we have clarified this point for the reviewer and future readers in~\fixRef{1.4.5}.
% 
Considering that the focus of this paper is a dataset release, we consider an analysis of neural network run-time performance to be outside of scope.
However, we have added in~\fixRef{1.4.7} (with a new reference in~\fixRef{1.4.8}) a note which will direct the interested reader to a paper listing exactly this information (processing time and memory footprint).
We have also in \fixRef{1.4.7} pointed the reader to our earlier work which does a run-time comparison between the radar-specific baselines presented. 
}

%------------------------------------------------------------------
\OB{1.5}{
Page 8 in the Result section: Regarding the results obtained using only a single nearest neighbor in the embedding space, have you explored varying the number of nearest neighbors? Could this potentially impact the final results?
}
%
\REP{1.5}{
We believe there has been a misunderstanding here.
\cref{fig:rc,tab:examples} both deal with nearest neighbour searches using more than a single nearest neighbour (all of $N=1$ to $N=10$ for~\cref{fig:rc} and $N=1,5,10$ for~\cref{tab:examples}).
The misunderstanding may be due to our phrasing on the indicated page, so we have updated that -- \fixRef{1.5}.
}

%------------------------------------------------------------------
\OB{1.6}{
Page 10 in the Conclusion section: it is recommended to quantify the results in the conclusion to provide a clearer overview of the findings.
}
\REP{1.6}{
We have amended the manuscript as suggested, \fixRef{1.6}.
}

%------------------------------------------------------------------
\OB{2.1}{
A concise description of the radar place recognition task, and its challenges should be given before directly presenting the relevant results.
}
%
\REP{2.1}{
The concise description of the radar place recognition task is as per \OB{3.1} below (please see \fixRef{3.1.2} for the change).
We have then also added a discussion of the challenges faced in this task -- please see \fixRef{2.1}.
}

%------------------------------------------------------------------
\OB{3.1}{
To better highlight the significance of the dataset, it would be beneficial to include a clear definition of place recognition and discuss its importance in applications such as robot navigation, SLAM, and autonomous driving. This will help readers understand the value of the presented dataset in the context of these research areas.
}
%
\REP{3.1}{
We have done as suggested -- \fixRef{3.1.1} and \fixRef{3.1.2}.
}

%------------------------------------------------------------------
\OB{3.2}{
The paper emphasizes the strengths of radar sensing, but it would be even more compelling to include experimental results comparing the performance of radar to other modalities like lidar or cameras in the given off-road scenarios. Since the dataset includes camera data, presenting comparative experimental results could further showcase the unique advantages of radar in these challenging environments.
}
%
\REP{3.2}{
Thank you for this suggestion.
We have run additional experiments using cameras, and have included the result in~\cref{fig:bfly_rc} (\fixRef{3.2.1}) and added a discussion (\fixRef{3.2.2}).
We believe that this suggestion has very much strengthened the paper, as it shows how the dataset can be used to confirm appearance-change robustness of radar as compared to the brittleness of camera in the face of these effects.
%
We have also added notes on the camera sensor specifications -- \fixRef{3.2.3}, with a new reference added in~\fixRef{3.2.4}.
%
Finally, we have summarised the camera data count in~\cref{tab:summary_table} -- \fixRef{3.2.5}.

Externally to the paper, we have processed and uploaded the camera images to the dataset website, \rurl{oxford-robotics-institute.github.io\\/oord-dataset}, e.g. for \texttt{2021-11-25-12-01-20} (\texttt{bellmouth}) linking to a Google Drive download at \rurl{drive.google.com/file/d/1Jy9oehCj59n92\\\_pDAS21yOSEkjm6JJPC/view} (all other routes/forays too).
}


%------------------------------------------------------------------
\OB{3.3}{
To ensure the reproducibility and usability of the dataset, it would be helpful to provide details on the extrinsic and intrinsic calibration between the radar, GPS/IMU, and camera sensors. This information is important for researchers interested in tasks like metric localization and sensor fusion.
}
%
\REP{3.3}{
We have measured and included these in the manuscript (\fixRef{3.3}) as well as in our software development kit (\rurl{github.com/mttgdd/oord-dataset/blob/\\main/config/extrinsics.yaml}).
}

%------------------------------------------------------------------
\OB{4.1}{
Present the figures in order as they appear in the text.
}
%
\REP{4.1}{
We believe the culprit here was~\cref{fig:dataset_overview_b} -- we have moved this into the correct order, see~\fixRef{4.1.2}.
We have also made sure that a few other floats appear \textit{after} the text that mentions them -- \cref{tab:vs_other_datasets} (\fixRef{4.1.2}) and \cref{fig:BFLY} (\fixRef{4.1.3}).
}

%------------------------------------------------------------------
\OB{4.2}{
Provide a caption for each figure/sub-figure.
}
%
\REP{4.2}{
We have added captions for every figure and subfigure -- please see \fixRef{4.2.1}, \fixRef{4.2.2}, \fixRef{4.2.3}, and \fixRef{4.2.4}.
}

%------------------------------------------------------------------
\OB{4.3}{
Figure 3 needs an axis labels.
}
%
\REP{4.3}{
We have updated the figure and added a note in the caption as per \fixRef{4.3}.
}

%------------------------------------------------------------------
\OB{4.4}{
Datasets can be referred to by a name rather than the data and time.
}
%
\REP{4.4}{
We have changed the way we reference the datasets, with the naming convention now \texttt{Route -- number}.
Please see \fixRef{4.4.1}, \fixRef{4.4.2}, \fixRef{4.4.3}, \fixRef{4.4.4}, and \fixRef{4.4.5}.
}

%------------------------------------------------------------------
\OB{4.5}{
Presented assessments on the dataset can be reorganized more technically. As it can be understood, the assessments are presented to highlight the versatile application of the dataset, and thus require a more concise storyline.
}
%
\REP{4.5}{
It is unclear if this review comment refers to organisation of~\cref{sec:examples} or~\cref{sec:results}.
%
In the case that the reviewer meant the former, we have now organised the baselines by type --
\fixRef{4.5.1}, \fixRef{4.5.2}, \fixRef{4.5.3}.
% 
In the case that the reviewer meant the latter, we have added organisational structure to this section -- \fixRef{4.5.4}, \fixRef{4.5.5}, \fixRef{4.5.8}.
We have also moved one block of text (\fixRef{4.5.6}) into a more appropriate location (\fixRef{4.5.7}).
}
